Content-Adaptive Pixel Discretization to Improve Model Robustness

Preprocessing defenses such as pixel discretization are appealing to remove adversarial attacks due to their simplicity. However, they have been shown to be ineffective except on simple datasets like MNIST. We hypothesize that existing discretization approaches failed because using a fixed codebook for the entire dataset limits their ability to balance image representation and codeword separability. We first formally prove that adaptive codebooks can provide stronger robustness guarantees than fixed codebooks as a preprocessing defense on some datasets. Based on that insight, we propose a content-adaptive pixel discretization defense called Essential Features, which discretizes the image to a per-image adaptive codebook to reduce the color space. We then find that Essential Features can be further optimized by applying adaptive blurring before the discretization to push perturbed pixel values back to their original value before determining the codebook. Against adaptive attacks, we show that content-adaptive pixel discretization extends the range of datasets that benefit in terms of both L_2 and L_infinity robustness where previously fixed codebooks were found to have failed. Our findings suggest that content-adaptive pixel discretization should be part of the repertoire for making models robust.

==> tex/tables/ablation_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!!]
\centering
\ifthenelse{\arxiv = 1}{\scriptsize}{}
\caption{Comparison between variants of \alg. All models are ATTA adversarially trained on the transform listed except for ImageNet, which use a pre-trained MAT model with the transform added at test time. * means that the most successful attack was a non-adaptive PGD attack, ** means that the most successful attack was a vanilla BPDA attack. Black-box numbers are with Square Attack.}\label{tab:variants}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{clccc}
\hline
\textbf{Dataset}                                                                  & \multicolumn{1}{c}{\textbf{Defense}} & \textbf{Accuracy} & \textbf{\begin{tabular}[c]{@{}c@{}}Robustness\\ (White-box)\end{tabular}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Robustness\\ (Black-box)\end{tabular}}} \\ \hline
\multirow{5}{*}{\textbf{MNIST}}                                                   & None                                 & 96.41\%           & 86.93\%                                                                   & 90.63\%                                                                                       \\
                                                                                  & EF - Full                            & 97.49\%           & 71.2\%                                                                    & 75.91\%                                                                                       \\
                                                                                  & EF - AB Only                         & 95.83\%           & 65.94\%                                                                   & 81.48\%                                                                                       \\
                                                                                  & \textbf{EF - AC Only}                & \textbf{98.56\%}  & \textbf{91.96\%}                                                          & \textbf{95.35\%}                                                                              \\
                                                                                  & EF - Gauss + AC                      & 98.13\%           & 69.13\%**                                                                 & 76.48\%                                                                                       \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fashion-\\ MNIST\end{tabular}}} & None                                 & 81.71\%           & 70.35\%                                                                   & 75.63\%                                                                                       \\
                                                                                  & EF - Full                            & 82.27\%           & 70.57\%                                                                   & 71.59\%                                                                                       \\
                                                                                  & EF - AB Only                         & 80.45\%           & 67.44\%                                                                   & 72.82\%                                                                                       \\
                                                                                  & \textbf{EF - AC Only}                & \textbf{82.48\%}  & \textbf{71.62\%*}                                                         & \textbf{72.87\%}                                                                              \\
                                                                                  & EF - Gauss + AC                      & 80.04\%           & 64.68\%**                                                                 & 67.22\%                                                                                       \\ \hline
\multirow{6}{*}{\textbf{CIFAR-10}}                                                & None                                 & 84.72\%           & 52.33\%                                                                   & 79.78\%                                                                                       \\
                                                                                  & EF - Full                            & 82.5\%            & 68.33\%**                                                                 & 49.5\%                                                                                        \\
                                                                                  & \textbf{EF - Full, FT}               & \textbf{79.44\%}  & \textbf{63.14\%**}                                                        & \textbf{57.47\%}                                                                              \\
                                                                                  & EF - AB Only                         & 85.88\%           & 52.86\%                                                                   & 80.92\%                                                                                       \\
                                                                                  & EF - AC Only                         & 86.06\%           & 53.18\%*                                                                  & 79.85\%                                                                                       \\
                                                                                  & EF - Gauss + AC                      & 86.98\%           & 31.4\%**                                                                  & 68.31\%                                                                                       \\ \hline
\multirow{5}{*}{\textbf{GTSRB}}                                                   & None                                 & 93.07\%           & 77.71\%                                                                   & 90.44\%                                                                                       \\
                                                                                  & \textbf{EF - Full}                   & \textbf{91.83\%}  & \textbf{78.59\%}                                                          & \textbf{87.18\%}                                                                              \\
                                                                                  & EF - AB Only                         & 92.92\%           & 78.33\%                                                                   & 90.79\%                                                                                       \\
                                                                                  & EF - AC Only                         & 92.19\%           & 78.23\%                                                                   & 88.48\%                                                                                       \\
                                                                                  & EF - Gauss + AC                      & 92.12\%           & 70.59\%**                                                                 & 84.84\%                                                                                       \\ \hline
\multirow{5}{*}{\textbf{RESISC45}}                                                & None                                 & 82.0\%            & 44.2\%                                                                    & 76.27\%                                                                                       \\
                                                                                  & \textbf{EF - Full}                   & \textbf{88.51\%}  & \textbf{66.73\%}                                                          & \textbf{73.02\%}                                                                              \\
                                                                                  & EF - AB Only                         & 85.93\%           & 41.8\%                                                                    & 80.53\%                                                                                       \\
                                                                                  & EF - AC Only                         & 83.49\%           & 47.04\%                                                                   & 76.69\%                                                                                       \\
                                                                                  & EF - Gauss + AC                      & 89.18\%           & 63.56\%                                                                   & 77.58\%                                                                                       \\ \hline
\multirow{5}{*}{\textbf{ImageNet}}                                                & None                                 & 97.23\%           & 5.32\%                                                                    & 97.24\%                                                                                       \\
                                                                                  & EF - Full                            & 89.47\%           & 18.49\%                                                                   & 89.63\%                                                                                       \\
                                                                                  & EF - AB Only                         & 93.55\%           & 8.60\%                                                                    & 93.60\%                                                                                       \\
                                                                                  & \textbf{EF - AC Only}                & \textbf{95.53\%}  & \textbf{22.59\%}                                                          & \textbf{95.59\%}                                                                              \\
                                                                                  & EF - Gauss + AC                      & 86.07\%           & 22.24\%                                                                   & 86.27\%                                                                                       \\ \hline
\end{tabular}
\end{table}

==> tex/tables/main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h!!]
\ifthenelse{\arxiv = 1}{\scriptsize}{}

\caption{Initial $L_\infty$ results. Generally, re-training on \alg has the highest robustness gains, particularly on RESISC45 which is a higher resolution dataset than the rest. Results from Chen et al. are reported directly from the original paper~\cite{chen2019towards} with the rows being selected on the basis of having the highest robustness floor except for MNIST (marked with *) where we found that PGD attack (non-adaptive to their transform) was more effective. On the various rows, * means that the most successful attack was a PGD attack (non-adaptive to the transform), ** means that the most successful attack was a vanilla BPDA attack. All asterisked lines are on small datasets. Best setting by robustness per dataset is bolded.}\label{tab:whitebox}
\centering
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}cllcccc@{}}
\toprule
\textbf{Dataset}                                                                  & \multicolumn{1}{c}{\textbf{Base Model}}             & \multicolumn{1}{c}{\textbf{Defense}} & \multicolumn{2}{c}{\textbf{Pre-trained}}                                        & \multicolumn{2}{c}{\textbf{Re-trained}}                                         \\
\multicolumn{1}{l}{}                                                              &                                                     &                                      & \multicolumn{1}{l}{\textbf{Accuracy}} & \multicolumn{1}{l}{\textbf{Robustness}} & \multicolumn{1}{l}{\textbf{Accuracy}} & \multicolumn{1}{l}{\textbf{Robustness}} \\ \midrule
\multirow{8}{*}{\textbf{MNIST}}                                                   & \multirow{3}{*}{Naturally Trained Model}            & None                                 & 99.24\%                               & 0\%                                     & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=2)                    & 98.81\%                               & 75.35\%                                 & 99.15\%                               & 80.91\%                                 \\
                                                                                  &                                                     & EF - AC Only                         & 99.12\%                               & 78.38\%                                 & 99.1\%                                & 80.89\%                                 \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{3}{*}{Adversarially Trained Model (MAT)}  & None                                 & 99.07\%                               & 93.23\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=2)                    & 98.93\%                      & 93.83\%*                        & 98.56\%                               & 92.80\%                                 \\
                                                                                  &                                                     & EF - AC Only                         & \textbf{98.95\%}                               & \textbf{93.86\%*}                                & \multicolumn{2}{c}{N/A}                                                         \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{2}{*}{Adversarially Trained Model (ATTA)} & None                                 & 96.41\%                               & 86.93\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF - AC Only                         & 96.05\%                               & 90.48\%*                                & 98.56\%                               & 91.96\%                                 \\ \midrule
\multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fashion-\\ MNIST\end{tabular}}} & \multirow{3}{*}{Naturally Trained Model}            & None                                 & 92.71\%                               & 1.6\%                                   & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=2)                    & 77.18\%                               & 38.07\%                                 & 86.74\%                               & 41.75\%                                 \\
                                                                                  &                                                     & EF - AC Only                         & 89.96\%                               & 38.78\%                                 & 90.27\%                               & 42.21\%                                 \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{3}{*}{Adversarially Trained Model (MAT)}  & None                                 & 87.63\%                               & 77.99\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=2)                    & 82.68\%                               & 66.52\%                                 & 86.18\%                               & 70.05\%                                 \\
                                                                                  &                                                     & EF - AC Only                         & \textbf{87.42\%}                      & \textbf{78.82\%*}                       & \multicolumn{2}{c}{N/A}                                                         \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{2}{*}{Adversarially Trained Model (ATTA)} & None                                 & 81.71\%                               & 70.35\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF - AC Only                         & 81.71\%                               & 72.68\%*                                & 82.48\%                               & 71.62\%                                 \\ \midrule
\multirow{8}{*}{\textbf{CIFAR-10}}                                                & \multirow{3}{*}{Naturally Trained Model}            & None                                 & 94.75\%                               & 2.23\%                                  & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=2)                    & 24.20\%                               & 15.90\%                                 & 68.50\%                               & 46.70\%                                 \\
                                                                                  &                                                     & EF (Ours)                            & 76.86\%                               & 47.36\%                                 & 90.93\%                               & 70.65\%                                 \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{3}{*}{Adversarially Trained Model (MAT)}  & None                                 & 87.14\%                               & 49.52\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=300)                  & 87.30\%                               & 46.90\%                                 & 86.80\%                               & 46.60\%                                 \\
                                                                                  &                                                     & EF (Ours)                            & 84.53\%                               & 47.35\%                                 & \multicolumn{2}{c}{N/A}                                                         \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{2}{*}{Adversarially Trained Model (ATTA)} & None                                 & 84.72\%                               & 52.33\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF (Ours)                            & 81.97\%                               & 51.69\%                                 & \textbf{82.5\%}                       & \textbf{68.33\%**}                      \\ \midrule
\multirow{8}{*}{\textbf{GTSRB}}                                                   & \multirow{3}{*}{Naturally Trained Model}            & None                                 & 95.36\%                               & 13.91\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=2)                    & 44.02\%                               & 23.94\%                                 & 55.39\%                               & 29.46\%                                 \\
                                                                                  &                                                     & EF (Ours)                            & 91.57\%                               & 30.86\%                                 & 94.44\%                               & 36.64\%                                 \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{3}{*}{Adversarially Trained Model (MAT)}  & None                                 & 93.68\%                               & 75.62\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & Chen et al. (k=500)                  & 93.98\%                               & 75.54\%                                 & 94.73\%                               & 76.66\%                                 \\
                                                                                  &                                                     & EF (Ours)                            & 90.30\%                               & 72.76\%                                 & \multicolumn{2}{c}{N/A}                                                         \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{2}{*}{Adversarially Trained Model (ATTA)} & None                                 & 93.07\%                               & 77.71\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF (Ours)                            & 89.72\%                               & 74.39\%                                 & \textbf{91.83\%}                      & \textbf{78.59\%}                        \\ \midrule
\multirow{6}{*}{\textbf{RESISC45}}                                                & \multirow{2}{*}{Naturally Trained Model}            & None                                 & 96.42\%                               & 0\%                                     & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF (Ours)                            & 57.44\%                               & 2.49\%                                  & 92.13\%                               & 4.18\%                                  \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{2}{*}{Adversarially Trained Model (MAT)}  & None                                 & 84.11\%                               & 40.07\%                                 & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF (Ours)                            & 61.76\%                               & 25.4\%                                  & \multicolumn{2}{c}{N/A}                                                         \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{2}{*}{Adversarially Trained Model (ATTA)} & None                                 & 82.0\%                                & 44.2\%                                  & \multicolumn{2}{c}{N/A}                                                         \\
                                                                                  &                                                     & EF (Ours)                            & 63.33\%                               & 29.87\%                                 & \textbf{88.51\%}                      & \textbf{66.73\%}                        \\ \midrule
\multirow{6}{*}{\textbf{ImageNet}}                                                & \multirow{3}{*}{Naturally Trained Model}            & None                                 & 94.71\%                               & 26.73\%                                 & \multicolumn{2}{c}{\multirow{3}{*}{N/A}}                                        \\
                                                                                  &                                                     & Chen et al. (k=300)                  & 89.30\%                               & 34.80\%                                 & \multicolumn{2}{c}{}                                                            \\
                                                                                  &                                                     & EF - AC Only                         & 92.32\%                               & 44.93\%                                 & \multicolumn{2}{c}{}                                                            \\ \cmidrule(l){2-7} 
                                                                                  & \multirow{3}{*}{Adversarially Trained Model (MAT)}  & None                                 & 97.23\%                               & 5.32\%                                  & \multicolumn{2}{c}{\multirow{3}{*}{N/A}}                                        \\
                                                                                  &                                                     & Chen et al. (k=500)                  & 94.80\%                               & 16.00\%                                 & \multicolumn{2}{c}{}                                                            \\
                                                                                  &                                                     & EF - AC Only                         & \textbf{95.53\%}                      & \textbf{22.59\%}                        & \multicolumn{2}{c}{}                                                            \\ \bottomrule
\end{tabular}
\vspace{-0.1in}
\end{table*}

==> tex/tables/square.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\caption{do asterisks add blackbox to square attack caption get rid of second rows highlight preferred technique}\label{tab:square}
\centering
\begin{tabular}{@{}cllccc@{}}
\toprule
\textbf{Dataset}                                                 & \textbf{Base Model}                & \multicolumn{1}{c}{\textbf{Defense}}                            & \textbf{Accuracy} & \textbf{\begin{tabular}[c]{@{}c@{}}Robustness\\ (White-box)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Robustness\\ (Square-Attack)\end{tabular}}      \\ \midrule
\textbf{MNIST}                                                   & Adversarially Trained Model (ATTA) & EF - K Only                                                     & 98.56\%           & 91.96\%                                                                   & \begin{tabular}[c]{@{}c@{}}97.84\% (100 steps)\\ 97.82\% (2000 steps)\end{tabular} \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Fashion\\ MNIST\end{tabular}} & Adversarially Trained Model (ATTA) & EF - K Only                                                     & 82.48\%           & 71.62\%*                                                                  & \begin{tabular}[c]{@{}c@{}}77.97\% (100 steps)\\ 75.42\% (2000 steps)\end{tabular} \\ \midrule
\textbf{CIFAR-10}                                                & Adversarially Trained Model (ATTA) & EF - Full                                                       & 82.5\%            & 68.33\%**                                                                 & \begin{tabular}[c]{@{}c@{}}49.5\% (40 steps)\\ 28.56\% (200 steps)\end{tabular}    \\ \midrule
\textbf{GTSRB}                                                   & Adversarially Trained Model (ATTA) & EF - Full                                                       & 91.83\%           & 78.59\%                                                                   & \begin{tabular}[c]{@{}c@{}}87.18\% (40 steps)\\ 82.24\% (200 steps)\end{tabular}   \\ \midrule
\textbf{RESISC45}                                                & Adversarially Trained Model (ATTA) & EF - Full                                                       & 88.51\%           & 66.73\%                                                                   & \begin{tabular}[c]{@{}c@{}}73.02\% (40 steps)\\ 55.38\% (200 steps)\end{tabular}   \\ \midrule
\textbf{ImageNet}                                                & Adversarially Trained Model (MAT)  & \begin{tabular}[c]{@{}l@{}}EF - Full,\\ pretrained\end{tabular} & 89.47\%           & 18.49\%                                                                   & \begin{tabular}[c]{@{}c@{}}89.63\% (10 steps)\\ 89.71\% (40 steps)\end{tabular}     \\ \bottomrule
\end{tabular}
\end{table*}
